Zero-Shot Automatic Pronunciation Assessment

Automatic Pronunciation Assessment (APA) is vital for computer-assisted language learning. Prior methods rely on annotated speech-text data to train Automatic Speech Recognition (ASR) models or speech-score data to train regression models. In this work, we propose a novel zero-shot APA method based on the pre-trained acoustic model, HuBERT. Our method involves encoding speech input and corrupting them via a masking module. We then employ the Transformer encoder and apply k-means clustering to obtain token sequences. Finally, a scoring module is designed to measure the number of wrongly recovered tokens. Experimental results on speechocean762 demonstrate that the proposed method achieves comparable performance to supervised regression baselines and outperforms non-regression baselines in terms of Pearson Correlation Coefficient (PCC). Additionally, we analyze how masking strategies affect the performance of APA.

==> Table/reg_results.tex <==
\begin{table}[htbp]
  \caption{Comparing the performance of various supervised baselines and unsupervised methods}
  \label{tab:example}
  \centering
  \begin{tabular}{ cccccccccccc }
    \toprule[1pt]
    \multicolumn{6}{c}{\textbf{Model}} & \multicolumn{6}{c}{\textbf{Speechocean762}} \\
    \hline
    \multicolumn{6}{c}{\textbf{Regression based}} & \multicolumn{6}{c}{}  \\
    \hline
    \multicolumn{6}{c}{GoP(SVR)}             &      \multicolumn{6}{c}{0.64}             \\
    \multicolumn{6}{c}{GoP(2BLSTM+MLP)}      &      \multicolumn{6}{c}{0.67}                 \\
    \multicolumn{6}{c}{DeepFeature}          &      \multicolumn{6}{c}{0.72}                \\
    \multicolumn{6}{c}{GOPT}                 &      \multicolumn{6}{c}{0.74}                \\

    \hline
    \multicolumn{6}{c}{\textbf{Non-regression based}} & \multicolumn{6}{c}{}  \\
    \hline
    \multicolumn{6}{c}{avgGoP}              &       \multicolumn{6}{c}{0.57}     \\
    \multicolumn{6}{c}{Ours}                &       \multicolumn{6}{c}{0.61}     \\
    \bottomrule[1pt]
  \end{tabular}
\end{table}


